Towards understanding how momentum improves generalization in deep learning

Stochastic gradient descent (SGD) with momentum is widely used for training modern deep learning architectures. While it is well-understood that using momentum can lead to faster convergence rate in various settings, it has also been observed that momentum yields higher generalization. Prior work argue that momentum stabilizes the SGD noise during training and this leads to higher generalization. In this paper, we adopt another perspective and first empirically show that gradient descent with momentum (GD+M) significantly improves generalization compared to gradient descent (GD) in some deep learning problems. From this observation, we formally study how momentum improves generalization. We devise a binary classification setting where a one-hidden layer (over-parameterized) convolutional neural network trained with GD+M provably generalizes better than the same network trained with GD, when both algorithms are similarly initialized. The key insight in our analysis is that momentum is beneficial in datasets where the examples share some feature but differ in their margin. Contrary to GD that memorizes the small margin data, GD+M still learns the feature in these data thanks to its historical gradients. Lastly, we empirically validate our theoretical findings.

==> rebuttal/message_ac.tex <==

We would like to bring to your attention some inconsistencies in review #2. Many critics in the review seem incorrect. For instance, the reviewer says that we are exaggerating in  our statements because we used the word "to address a question" in the introduction. Indeed, the reviewer seems to confuse the words "to address" and "to solve". In the paper, we have never claimed that we solved the question "why momentum improves generalization in deep learning?" and in the introduction, we clearly state the result for a two-layer neural network for a specific dataset.   Besides, the reviewer finds the numerical results "unconvincing" because we run our  CIFAR-10 experiments for 300 epochs and not for "1200 epochs". We are confused by this since in several optimization papers  ([1,2,3] among many others) these experiments are run for 200-250 epochs. Lastly, in all our experiments (e.g. see Figure 1), we make sure that the train loss is smaller than 1e-3 (it cannot be zero due to weight decay) and that the training accuracy is > 99.9\%.  For these reasons, we do not think that reviewer 2 depicts a fair evaluation of our work.


[1] Agarwal, R. A., et al. (2020). Disentangling adaptive gradient methods from learning rates.

[2] Foret, P., et al. (2020). Sharpness-aware minimization for efficiently improving generalization.

[3] Gupta, V., et al. (2018). Shampoo: Preconditioned stochastic tensor optimization.

==> rebuttal/momentum_rebuttal.tex <==
We thank the reviewers for their insightful comments. We are glad that the reviewers found that the addressed question is  "very important'' 
(\Rthree, \Rfour) and our contribution "novel" (\Rthree, \Rfour). We are also heartened to hear that \Rtwo\ found our setting ``significant'' and that \Rthree, \Rfour\ described our analysis as "well-written" and "clear".

%We address reviewers concerns in order R4-R3-R2. Due to space limitation, we only focus on the most critical comments.
% We will address all comments in the final version.





\textbf{\Rtwo-\Rthree: "mechanism does not appear in practice", "only mechanism?"}

First, we believe that this mechanism do appear in practice through the two experiments. Figure 3 shows that in the synthetic setting where we artificially create small and large margin data, GD+M classifies better the small margin data compared to GD. In Figure 4, we take a real-world dataset (CIFAR-10) and create small margin data by decimating some images. We see that GD+M is able to well-classify these decimated images compared to GD. Small margin data appear naturally in CIFAR-10 since if we look at the dataset, some images are hard to distinguish for a human. However, it is not feasible to ask a human to hand-annotate whether the 50000 images are blurry or not. Thus, we opted for the proxy of creating small margin data by decimating images. Lastly, we admit that we do not know whether this is the only mechanism appearing in practice. As acknowledged by the reviewers, our work is among the first on this question and we hope that it will lead to the discovery other mechanisms.




\textbf{\Rfour: choice of cubic activation and why our analysis is insightful for general case}

We first acknowldege that our setting and choice of the cubic activation is specific. However, there are multiple points we would like to clarify. First, the scientific process in deep learning theory is typically as follows: we first conduct experiments on real-world data sets and models, observe a phenomenon and then come up with a simplified model/data set to prove this phenomenon. Now we want to clarify our choice of cubic activation. We are confused by the landscape argument brought by the reviewer. Following this logic, an important number of seminal works in deep learning (including [3], previous best paper runner up in ICML)  have limited relevance. Indeed, [1] shows that deep linear networks have no spurious local minima.  Yet, [2] and [3] respectively use deep linear networks to study batch normalization and representation learning. Similarly, [4] shows on quadratic networks that depending on the scale of initialization, the solution towards GD converges is different. Thus, the first point we make is that similarly to the aforementioned papers, we use neural network with cubic activations as a simplified setting to study momentum. Secondly, neural networks with polynomial activations numerically perform well: wideresnets with quadratic activations compete those with ReLU on CIFAR-10 [5]. Lastly, we do \textit{theoretically} and \textit{numerically} (Figure 3) prove that in our setting with cubic activations, GD and GD+M converge to different \emph{local optimal} solutions even when adding weight decay. Therefore, in our setting with cubic activation the landscape has spurious local minima. To conclude, we believe that our setting is insightful as we demonstrate that there are multiple local minima and GD and GD+M converge to two different minima. We agree with the reviewer that the generalization improvement by momentum may be a more general property related to the structure of the loss and the dataset. However, our work is the first investigating this question and we hope it to be a first step to understand this phenomenon. %If we want to make progress in theory of deep learning, those first steps should not be discouraged. 


\textbf{\Rthree: "Focus on GD rather than SGD"}

We analyze GD instead of SGD because: (1). The gap between momentum and without momentum grows with increasing batch size (see Figure 6(a)). (2). It isolates the generalization effect induced by momentum since it has been observed that SGD noise affects generalization. From a practical view, SGD with very large batch-size (which corresponds to GD) is used in huge vision models e.g. BiT. Lastly, we believe that understanding momentum in GD is useful to understand it for SGD.


\textbf{\Rthree: "Simpler setting" }

A potential simpler setting may be our setting with $d = 1$. However, our proof only works for sufficiently large $d$ (so the network can memorize noise). We don't think it can be extended to the setting mentioned by the reviewer. 
%\textcolor{red}{Yuanzhi: I don't really know what to say about the general theory based on land}

%We acknowledge that the appendix is long. However, we did our best to include all the details so that a unexperienced reader understands the proofs. For the sake of brevity, we could easily remove 30 pages but the paper would be harder to read. Length of the paper,  

\textbf{\Rtwo: "Presentation of contributions [...] exaggerated"}

To our knowledge, ``address a question" means ``to deal with it, but not necessarily solve it". Nowhere in the paper we claim that we completely solve why momentum improves generalization.  In the introduction, we  say that  our theorem is only for two-layer neural network on specific data set. 

%We will ensure in the final version that there is no overstatements. 
%Nowhere in the paper we claim that we completely solve why momentum improves generalization. 

\textbf{\Rtwo: "Lower end number of epochs"}

Several seminal papers as [6] train Resnets on CIFAR-10 for 200-250 epochs. This is why we opted for 300 epochs. In all of our experiments, the training loss is always below 1e-3 (they cannot be zero due to weight decay), and the training accuracies are $> 99.9\%$. We repeated the same experiment as Figure 1 for 1000 epochs. Train loss (GD): 3e-4; (GD+M): 9e-4. Test accuracy (GD): 72.03\%; (GD+M): 83.08\%. Conclusions are same even with longer training. 



[1] Kawaguchi. Deep learning without poor local minima.


[2] Santurkar, S., et al. (2018). How does batch normalization help optimization?

[3] Tian, Y., et al. (2021). Understanding self-supervised learning dynamics without contrastive pairs

[4] Woodworth, B., et al. (2020). Kernel and rich regimes in overparametrized models.

[5] Allen-Zhu, Z., \& Li, Y. (2020). Backward feature correction: How deep learning performs deep learning.

%[6] HaoChen, J. Z., et al. (2021). Shape matters: Understanding the implicit bias of the noise covariance.

%[7] Kolesnikov, A., et al. (2020). Big transfer (bit): General visual representation learning.

[6] Foret, P., et al. (2020). Sharpness-aware minimization for efficiently improving generalization.




==> rebuttal/old_rebuttal.tex <==
We thank the reviewers for their insightful comments. We are glad that the reviewers found that the addressed question is  "very important'' 
(\Rthree, \Rfour) and our contribution "novel" (\Rthree, \Rfour). We are also heartened to hear that \Rtwo\ found our setting ``significant'' and that \Rthree, \Rfour\ described our analysis as "well-written" and "clear".

%We address reviewers concerns in order R4-R3-R2. Due to space limitation, we only focus on the most critical comments.
% We will address all comments in the final version.





\textbf{\Rtwo-\Rthree: "mechanism does not appear in practice", "only mechanism?"}

First, we believe that this mechanism do appear in practice through the two experiments. Figure 3 shows that in the synthetic setting where we artificially create small and large margin data, GD+M classifies better the small margin data compared to GD. In Figure 4, we take a real-world dataset (CIFAR-10) and create small margin data by decimating some images. We see that GD+M is able to well-classify these decimated images compared to GD. Small margin data appear naturally in CIFAR-10 since if we look at the dataset, some images are hard to distinguish for a human. However, it is not feasible to ask a human to hand-annotate whether the 50000 images are blurry or not. Thus, we opted for the proxy of creating small margin data by decimating images. Lastly, we admit that we do not know whether this is the only mechanism appearing in practice. As acknowledged by the reviewers, our work is among the first on this question and we hope that it will lead to the discovery other mechanisms.




\textbf{\Rfour: choice of cubic activation and why our analysis is insightful for general case}

We first acknowldege that our setting and choice of the cubic activation is specific. However, there are multiple points we would like to clarify. First, the scientific process in deep learning theory is typically as follows: we first conduct experiments on real-world data sets and models, observe a phenomenon and then come up with a simplified model/data set to prove this phenomenon. Now we want to clarify our choice of cubic activation. We are confused by the landscape argument brought by the reviewer. Following this logic, an important number of seminal works in deep learning (including [3], previous best paper runner up in ICML)  have limited relevance. Indeed, [1] shows that deep linear networks have no spurious local minima.  Yet, [2] and [3] respectively use deep linear networks to study batch normalization and representation learning. Similarly, [4] shows on quadratic networks that depending on the scale of initialization, the solution towards GD converges is different. Thus, the first point we make is that similarly to the aforementioned papers, we use neural network with cubic activations as a simplified setting to study momentum. Secondly, neural networks with polynomial activations numerically perform well: wideresnets with quadratic activations compete those with ReLU on CIFAR-10 [5]. Lastly, we do \textit{theoretically} and \textit{numerically} (Figure 3) prove that in our setting with cubic activations, GD and GD+M converge to different \emph{local optimal} solutions even when adding weight decay. Therefore, in our setting with cubic activation the landscape has spurious local minima. To conclude, we believe that our setting is insightful as we demonstrate that there are multiple local minima and GD and GD+M converge to two different minima. We agree with the reviewer that the generalization improvement by momentum may be a more general property related to the structure of the loss and the dataset. However, our work is the first investigating this question and we hope it to be a first step to understand this phenomenon. %If we want to make progress in theory of deep learning, those first steps should not be discouraged. 


\textbf{\Rthree: "Focus on GD rather than SGD"}

We analyze GD instead of SGD because: (1). The gap between momentum and without momentum grows with increasing batch size (see Figure 6(a)). (2). It isolates the generalization effect induced by momentum since it has been observed that SGD noise affects generalization. From a practical view, SGD with very large batch-size (which corresponds to GD) is used in huge vision models e.g. BiT. Lastly, we believe that understanding momentum in GD is useful to understand it for SGD.


\textbf{\Rthree: "Simpler setting" }

A potential simpler setting may be our setting with $d = 1$. However, our proof only works for sufficiently large $d$ (so the network can memorize noise). We don't think it can be extended to the setting mentioned by the reviewer. 
%\textcolor{red}{Yuanzhi: I don't really know what to say about the general theory based on land}

%We acknowledge that the appendix is long. However, we did our best to include all the details so that a unexperienced reader understands the proofs. For the sake of brevity, we could easily remove 30 pages but the paper would be harder to read. Length of the paper,  

\textbf{\Rtwo: "Presentation of contributions [...] exaggerated"}

To our knowledge, ``address a question" means ``to deal with it, but not necessarily solve it". Nowhere in the paper we claim that we completely solve why momentum improves generalization.  In the introduction, we  say that  our theorem is only for two-layer neural network on specific data set. 

%We will ensure in the final version that there is no overstatements. 
%Nowhere in the paper we claim that we completely solve why momentum improves generalization. 

\textbf{\Rtwo: "Lower end number of epochs"}

Several seminal papers as [6] train Resnets on CIFAR-10 for 200-250 epochs. This is why we opted for 300 epochs. In all of our experiments, the training loss is always below 1e-3 (they cannot be zero due to weight decay), and the training accuracies are $> 99.9\%$. We repeated the same experiment as Figure 1 for 1000 epochs. Train loss (GD): 3e-4; (GD+M): 9e-4. Test accuracy (GD): 72.03\%; (GD+M): 83.08\%. Conclusions are same even with longer training. 



[1] Kawaguchi. Deep learning without poor local minima.


[2] Santurkar, S., et al. (2018). How does batch normalization help optimization?

[3] Tian, Y., et al. (2021). Understanding self-supervised learning dynamics without contrastive pairs

[4] Woodworth, B., et al. (2020). Kernel and rich regimes in overparametrized models.

[5] Allen-Zhu, Z., \& Li, Y. (2020). Backward feature correction: How deep learning performs deep learning.

%[6] HaoChen, J. Z., et al. (2021). Shape matters: Understanding the implicit bias of the noise covariance.

%[7] Kolesnikov, A., et al. (2020). Big transfer (bit): General visual representation learning.

[6] Foret, P., et al. (2020). Sharpness-aware minimization for efficiently improving generalization.



